Optimal (Randomized) Parallel Algorithms in the Binary-Forking Model

In this paper we develop optimal algorithms in the binary-forking model for a variety of fundamental problems, including sorting, semisorting, list ranking, tree contraction, range minima, and ordered set union, intersection and difference. In the binary-forking model, tasks can only fork into two child tasks, but can do so recursively and asynchronously. The tasks share memory, supporting reads, writes and test-and-sets. Costs are measured in terms of work (total number of instructions), and span (longest dependence chain). The binary-forking model is meant to capture both algorithm performance and algorithm-design considerations on many existing multithreaded languages, which are also asynchronous and rely on binary forks either explicitly or under the covers. In contrast to the widely studied PRAM model, it does not assume arbitrary-way forks nor synchronous operations, both of which are hard to implement in modern hardware. While optimal PRAM algorithms are known for the problems studied herein, it turns out that arbitrary-way forking and strict synchronization are powerful, if unrealistic, capabilities. Natural simulations of these PRAM algorithms in the binary-forking model (i.e., implementations in existing parallel languages) incur an $\Omega(\log n)$ overhead in span. This paper explores techniques for designing optimal algorithms when limited to binary forking and assuming asynchrony. All algorithms described in this paper are the first algorithms with optimal work and span in the binary-forking model. Most of the algorithms are simple. Many are randomized.

==> app-figure.tex <==
\begin{figure}[t]
\vspace{-.5em}
\begin{center}
  \includegraphics[width=\columnwidth]{figures/tree}
\end{center}\vspace{-1.2em}
\caption{\label{fig:tree} An example of the tree contraction algorithm.  It first generates the priority of the leaf node from a random permutation, as shown in Figure~(a).
Then every interior node computes the highest priority label in the subtree, and the computed values are shown as the blue numbers in Figure~(b).
Then each interior node $v$ is paired with the leave node that has the priority which is stored in the child node different from the priority of $v$.
Taking the root node as an example, the priority 5 is different from the right node which has priority 4, so the root node is paired with the leaf node with priority 4.
The pairing results are shown as the red numbers in Figure~(c).
In this example, leaf nodes 0, 1, and 2 can be contracted simultaneously, and the contracted tree is shown in Figure~(d).
}

\bigskip

\begin{minipage}[t]{\columnwidth}
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/treepath.pdf}
    \caption{An illustration about adjusting red nodes in Proof \ref{lem:uppers}. (a) Extend all inner joint nodes to some external node. (b) Move all joint nodes to upper levels as far as possible. (c) The final shape after adjusting the red nodes.  All joint nodes are at the top, and all linking nodes form chains at bottom.}\label{fig:treepath}
\end{minipage}
\end{figure}

\begin{figure}
\begin{minipage}[t]{\columnwidth}
    \centering
  \includegraphics[width=\columnwidth]{figures/treealgorithm.pdf}
  \caption{An illustration of the set-set algorithms. We first split both trees into \tchunk{s} by the glaobally $b$-th, $2b$-th, ..., elements. Here $b=\frac{m+n}{4}$, but in general $b$ should be $O(\sqrt{m+n})$. We then recursively sketch each pair of \tchunk{s}, until we reach the base case and call the base case algorithms (see Figure \ref{fig:basecase}). We then connect the results with pivots, and get the \emph{sketch} of the result tree. Finally we rebalance the tree structure and fill in all tombs.}\label{fig:setalgorithm}
\end{minipage}

\bigskip
  \includegraphics[width=.9\columnwidth]{figures/base-tree.pdf}
  \caption{Illustrations for the base case algorithms for \union{}, \intersection{} and \difference{}. Objects in $T_L$ are marked in blue, and objects in $T_S$ are marked in yellow.}\label{fig:basecase}

\end{figure}




==> app-set.tex <==
\section{Proof Details of Lemma~\ref{lem:uppers}, \ref{lem:sumbound}, \ref{lem:mpivots} and \ref{lem:step1height} for Ordered Set-Set Operations}
\label{app:setproof}










==> app-sort.tex <==
\section{Cost Bounds for the Distribution Step}
\label{app:sort}

Here we supply more algebraic details of the cost analysis for the distribution step and show the following lemma.

\begin{lemma}
The distribution step as mentioned in Section~\ref{sec:sorting} has $O(n'(\log n'+\log n / \log \log n))$ work and $O(\log n'+\log n / \log \log n)$ depth \whp{} for subproblem size $n'$ and overall input size $n$.
\end{lemma}
\begin{proof}
  The possibility that a random position is empty is at least $1-1/d$, and the retry chance is less than $1/d$.
  The possibility for $c'd$ consecutive retries is:
  \begin{eqnarray*}
  d^{-c'd} &=& \left(\frac{\log_2 \log_2 n}{\log_2 n}\right)^{\frac{c'\log_2 n}{\log_2 \log_2 n}}\\
  &<& \left(\left(\log_2 n\right)^{\log_2 \log_2 n}\right)^{-\frac{c'\log_2 n}{2}}\qquad(*)\\
  &=& 2^{-\frac{c'\log_2 n}{2}} ~=~ n^{-c'/2}
\end{eqnarray*}
In (*) we assume that
The depth bound is hence $\log_2 n'+O(d)=O(\log n'+\log n / \log \log n)$ \whp{}.
The work for the comparisons between the elements and the pivots is $O(n'\log \sqrt{n'})=O(n'\log n')$.
The work of finding the locations and packing the lists is $O(dn')$ \whp{}.
Summing the two costs gives the stated work bound.
\end{proof}

\hide{
\begin{proof}
  By setting the base case size $\delta=\log_2^6 n$ and using an arbitrary parallel sorting algorithm for the base case (e.g., the trivial parallel mergesort~\cite{blelloch2010low}), any subproblem with size $n'\le \delta$ uses $O(n'\log n')$ work and $O(\log^2 \log n')$ depth.
  Assuming the distribution step (line~\ref{line:distribution}) takes $W_{\smb{dis}}(n')$ expected work and $D_{\smb{dis}}(n')$ depth \whp{}, we have the following recurrences for the cost bounds:
  \begin{eqnarray*}
  W(n')&\le& (n')^{1/3}W((n')^{2/3})+O(n')+W_{\smb{dis}}(n')\\
  D(n')&\le& D((n')^{2/3})+O(\log n')+D_{\smb{dis}}(n')
  \end{eqnarray*}
  Here we pessimistically assume that $q=(n')^{1/3}$ which can only be achieved when $n'=\Theta(\log^6 n)$.
  This is the worst-case and shown in the recurrences, and in practice it can only be better.
  The recurrence depth is $O(\log \log n)$, so if $W_{\smb{dis}}(n')$ and $D_{\smb{dis}}(n')$ are $O(n'(\log n'+\log n / \log \log n))$ and $O(\log n'+\log n / \log \log n)$ respectively, then
  plugging in the base case cost gives the stated bounds in the theorem.
  We will discuss how to achieve the bounds of the distribution step (line~\ref{line:distribution}) in the next paragraph.

  When the $q$ pivots have been decided, we generate $q+1$ lists for the buckets each with size $c'dn'/q$, where $d=c\log n/\log \log n$.
  By setting $c'$ correctly, we can guarantee the list size is $d$ times large than the number of elements in the bucket \whp{} (Chernoff bound).
  Then we apply a parallel for-loop for every element, and use a binary search for each element to decide the corresponding bucket.
  Then each element will iteratively select a random position in the list, try to \TAS{} to reserve the position, and redo this process if it fails.
  After all elements are inserted, we pack the lists to get the partition of the input elements.
  The number of retries of each element is bounded by $O(d)$ \whp{}, which gives the desired work and depth bounds.
  More algebraic details are provided in Appendix~\ref{app:sort-bound}.
\end{proof}

}



==> models.tex <==
\section{The Model and Simulations}
\label{sec:mtram}

\newcommand{\tram}{TRAM}

Here we describe the \bfmodel{} and its relationship to more
traditional models of parallel computing, including the PRAM and
circuit models.  The \bfmodel{} falls into the class of multithreaded
models~\cite{blumofe1999scheduling,BGM99,ABP01,CR17b,BL98}.
Multithreaded computational models assume a collection of threads
(sometimes called processes or tasks) that can be dynamically created,
and generally run asynchronously.  Cost is determined in terms of the
total work and the computational span (also called depth or critical
path length).  There are several variants on multithreaded models depending on
how many threads can be forked, how they synchronize, and assumptions
about how the memory can be accessed.

For the purpose of being concrete, we define specific models in this
paper based on the models described in the references above.  We start
by defining a more general model, the \tram{} (tee-ram), that allows arbitrary
forking and then define the \bfmodel{} as a special case.

\paragraph{\tram.}

The \defn{Threaded Random-Access Machine
  (\tram{})} %~\cite{blelloch18notes}
consists of a set of \defn{\thread{}s} that share a common memory.
Each \thread{} acts like a sequential RAM---it works on a program
stored in the shared memory, has a constant number of registers, and
has standard RAM instructions (including an \insend{} to finish the
computation).  The \tram{} extends the RAM with a \forkins{}
instruction that takes a positive integer $k$ and forks $k$ new child
\thread{}s.  Each child \thread{} receives a unique integer in the
range $1,\ldots,k$ in its first register and otherwise has the
identical state as the parent, which has a $0$ in that register.  The
children all start by running the next instruction.  When a \thread{}
performs a \forkins{}, it is suspended until all the children
terminate (execute an \insend{} instruction).  The first instruction
run by the parent when all its children complete is called a
\defn{join} instruction.  A computation starts with a single
\defn{root} \thread{} and finishes when that root \thread{} ends.
This model supports what is often referred to as nested parallelism.
If the root \thread{} never does a fork, it is a standard sequential
program.  As is standard with the sequential RAM~\cite{Tarjan83}, we
assume that for an input of size $n$, all memory locations and
registers can hold $O(\log n)$ bits.  This prevents hiding unbounded
parallelism within single instructions and is an accurate
representation of real machines.

A computation in the \tram{} defines a partial order on the
instructions.  In particular, (1) every instruction depends on its previous
instruction in the same \thread{} (if any), (2) every first instruction in a
thread depends on the fork instruction of the parent that generated
it, and (3) every join instruction depends on the \insend{} instruction of all
child \thread{}s that the corresponding fork generated.  These
dependences define the partial order.  The \emph{work} of a
computation is the total number of instructions, and the \emph{\spanc{}}
is the longest sequence of dependent instructions.  As usual, the
partial order can be viewed as a DAG.

We assume that the results of memory operations are consistent with
some total order (linearization) on the instructions that preserves
the partial order---i.e., a read will return the value of the previous
write to the same location in the total order.  The choice of total
order can affect the results of a program since \thread{}s can
communicate through the shared memory.  In general, therefore,
computations can be nondeterministic.  Two instructions are said to be
\defn{concurrent} if they are unordered, and \defn{ordered} otherwise.
Two instructions \emph{conflict} if one writes to a memory location
that the other reads or writes.  We say two
instructions \defn{race} if they are concurrent and conflict.  If
there are no races in a computation, then all linearized orders will
return the same result.   A particular linearized order is to iterate
sequentially from the first to last child in each fork.  We call this
the \defn{sequential ordering}.
The new algorithms for range minimum query and set operations in this paper are race-free, and the others are not.

Since the \tram{} is asynchronous, it can be useful to add some
additional memory instructions for the purpose of synchronizing.
Possible instructions include \texttt{test-and-set} (\texttt{TS}),
\texttt{fetch-and-add} (\texttt{FA}), \texttt{compare-and-swap}
(\texttt{CAS}), and \texttt{priority-write} (\texttt{PW}).  In this
paper we use \texttt{TS}, which takes a reference to a memory
location, and atomically checks if its contents is 0 and if so sets it
to 1 and returns \texttt{true}; otherwise it returns \texttt{false}.
To simplify issues of parallel memory allocation we assume an
\allocateins{} instruction that takes a positive integer $n$ and
allocates a contiguous block of $n$ memory locations, returning a
pointer to the block, and a \freeins{} instruction that given a
pointer to an allocated block, frees it.

\paragraph{The \bfmodel.}

The \defn{\bfmodel{}} is the \tram{} with $k = 2$, i.e, it only
directly supports binary forking, and supporting \texttt{TS}.  From an
asymptotic point of view, any constant forking is equivalent.
However, allowing to fork based on a variable in a register or a
function of input size is not equivalent.  Nevertheless, it is
convenient to express algorithms with $k$-way forks, for $k>2$; in the
\bfmodel{} large-way forks in the algorithm description are treated as
syntactic sugar for a $\lg(k)$-height tree of forks.

The motivation for the binary-forking variant of the \tram{} model and
for using the \texttt{TS} primitives is based on both theoretical and
practical considerations.  From a theoretical perspective, it allows
strong simulation bounds for the model on the PRAM and on other more
loosely coupled processor models.  In particular, as described in more
detail below, the \bfmodel{} with \texttt{TS} can be simulated
optimally on these machines, at least assuming randomization, and
\whp{}.  This is not known to be true for the non-constant forking,
nor is it known if we add more powerful memory primitives such
as~\texttt{CAS}.  Another nice theoretical property of binary forking
with \texttt{TS} is that it can be simulated with no loss in a weaker
model that assumes the parent thread never continues---i.e., when both
children finish, that subcomputation is done.  Continuing the parent
can be simulated by having the child that finishes later take
over the parent.  The \texttt{TS} can be used to determine which is
later.   In fact we know of no way to efficiently implement a join on an
asynchronous machine that does not use a primitive as powerful as
the \texttt{TS} instruction.        

From a practical perspective, most implementations of multithreading
are based on
binary-forking~\cite{blelloch1992nesl,frigo1998implementation,Java-fork-join,OpenMP,charles2005x10,budimlic2011design,TBB,TPL}.
Some of these have parallel loops of arbitrary size (arbitrary-way
forking), but they are implemented using binary forking by creating a
tree of forks.  Furthermore all machines today support \texttt{TS},
and experimental analysis has shown that it is as efficient as reads
and writes even under high contention~\cite{SBFG13}.

Finally, we note that \texttt{TS} is important for some of our
algorithms.  It is an interesting question for future work whether it
is really necessary, or whether the other memory primitives can
significantly help for other problems, or perhaps to derandomize
our algorithms.

We use $\mathcal{BF}(W(n),S(n))$ to denote the class of algorithms that require
$O(W(n))$ work and $O(S(n))$ span for inputs of size $n$ in the \bfmodel{}.
Similarly we use $\TRAM(W(n),S(n))$ for the \tram{}
model with arbitrary forking.
We use
$\mathcal{BF}^k$ ($\TRAM^k$) when $S(n) = O(\log^k(n))$ and $W(n)$ is
polynomial in $n$, and
$\mathcal{BF}^*$ ($\TRAM^*$) when the span is polylogarithmic and the
work is polynomial.


\paragraph{PRAM.}

For background, we give a brief description of the PRAM
model~\cite{SV81}.  A PRAM consists of $p$ processors, each a sequential
random access machine (RAM), connected to a common shared memory of
unbounded size.  Processors run synchronously in lockstep.  Although
processors have their own instruction pointer, in typical algorithms
they all run the same program.  There are several variants of the
model depending on how concurrent accesses to shared memory are
handled---e.g., CRCW allows concurrent reads and writes, and EREW
requires exclusive reads and writes.  For concurrent writes, in this
paper we assume an arbitrary element is written (the most standard
assumption).  A more detailed description of the model and its
variants can be found in J\'{a}J\'a's book on parallel
algorithms~\cite{JaJa92}.  As with the TRAM, we assume that for an
input of size $n$, memory locations and registers contain at most
$O(\log n)$ bits.   We use
$\PRAM(W(n),S(n))$ to indicate PRAM algorithms that run in $O(W(n))$
work (processor-time product) and $S(n)$ time,
$\PRAM^k$ when the time is $O(\log^k n)$, and
$\PRAM^*$ when it is polylogarithmic (both with polynomial work).

A crucial difference between the PRAM from the TRAM is the fact that
the latter is asynchronous.  If two large (possibly
parallel) tasks are forked in the \tram, it is perfectly valid to
fully execute the first, and later the second, or the other way round,
or interleave their instructions in any arbitrary way that satisfies
the dependences.  Another difference is the ability to fork new
threads.

%Given the differences it is important to understand the
%relationship between the two classes of models.

\paragraph{Relationship to the PRAM.}

There have been many scheduling results showing how to schedule
\tram{}, and multiway forking on various machine
models~\cite{blumofe1999scheduling,BGM99,ABP01}.  For example, the
following theorem can bound the runtime for programs
in the \bfmodel{} on a $P$ processor loosely synchronized parallel
machine.

\begin{theorem}[\cite{BL98}]
  \label{thm:workstealing}
  For any computation in the \bfmodel{} that does $W$ work and has $D$
  span, can be simulated on $P$ processors of a loosely synchronous
  parallel machine or the CRCW PRAM in \[O\left(\frac{W}{P}+D\right)\]
  time \whp{} in $W$.
\end{theorem}

\noindent
This is asymptotically optimal (modulo randomization) since the
simulation must require the maximum of $W/P$ (assuming perfect balance
of work) and $D$ (assuming perfect progress along the critical path).
The result is based on a work-stealing scheduler.  A slight variant of
the theorem applies in a more general setting where individual
processors can stop and start~\cite{ABP01} and $P$ is the average
number of processors available.  It is easy to extend the above
theorem for the arbitrary-CRCW model to include \texttt{TS}.  In
particular, in a constant-length sequence of synchronous step, all
processors can (1) check if the location is already set, (2) if not,
write their processor number to the location, and (3) read it back to
see if they won.

The best that is known for simulating the \tram{} with arbitrary $k$
on a $p$-processor CRCW PRAM is
\[O\left(\frac{W}{P}+D \log^{*} p \right),\]
also randomized~\cite{BGM99}.    This is based on using
approximate prefix sums~\cite{Goodrich94}.

Simulating in the other direction, a $p$-processor CRCW PRAM can be trivially
simulated on the \tram{} with $k = p$ with no loss in work or span.
Importantly, however, simulating a $p$-processor PRAM, even the
weakest EREW version, on the \bfmodel{} requires a $\Theta(\log p)$
factor loss in span.  This is a lower bound for any simulation that is
faithful to the synchronous steps since just forking $p$ parallel
instructions (one step on a PRAM) requires at least $\log p$ steps on
the \bfmodel.

\paragraph{Relationship to Circuit Models.}
Beyond the PRAM we can ask about the relationship to circuit models and to
bounded space.  Here we use $\NC$ for Nick's class, $\AC$ when allowing
unbounded in-degree, and $\LogSpace$ for logspace~\cite{Borodin77,KarpR90}.  We first
note that $\NC = \BF^* = \TRAM^*$.  This follows directly from the
PRAM simulations since
$\NC = \PRAM^*$~\cite{KarpR90}.    We also have the following
more fine-grained results.

\begin{theorem}
\[ \NC^1 \subseteq \LogSpace \subseteq \BF^1 \subseteq \AC^1 = \PRAM_{CRCW}^1 \subseteq \TRAM^1 \subseteq \NC^2 \]
\end{theorem}
\begin{proof}
(Outline).   The first inclusion is well known~\cite{Borodin77}.
% Simulating an $\NC^1$ circuit in $\BF^1$ (without \texttt{TS}) is
% straightforward.  We start at the output bit and follow backwards
% forking two child threads for each of the two inputs.  Since the
% circuit is $O(\log n)$ deep, we will only fork off polynomially many
% threads, limiting the work to $O(n^k)$.
To simulate $L$ in $\BF^1$ we can construct a graph representing the
state transition diagram of the logspace computation.  Each state
looks at one bit of the input tape and has two edges out, one for 0
and one for 1.  The construction is logspace uniform.  For a
particular input of length $n$ we select the appropriate edges, which
forms a forest with the accept states appearing as some of the roots.
An Euler Tour can be built on the trees in the forest---not hard to do
in logarithmic span.  Using deterministic list-contraction, as
described at the end of the next section, the simulation can identify
if the start state has an accept state as its root.  The full
computation has $O(\log n)$ span and does polynomial work (there are
polynomially many states).

To simulate $\BF^1$ in $\AC^1$ we could use
know results for simulating the CRCW PRAM in circuit depth
proportional to time~\cite{ChandraSV84}, but this would require randomization
since our simulation of the \bfmodel{} on the PRAM uses
randomization.  However, it is not difficult to extend the ideas for a
deterministic simulation.  The idea is that the shared memory can be
simulated in constant depth per step~\cite{KarpR90}, as can the processor.
The processor simulation can take advantage of the fact that our registers only
have $O(\log n)$ bits and instructions only take a constant number of
registers.  This allows instructions to be simulated in constant
depth and polynomial size, effectively by table lookup (just index the
correct solution based on the $O(\log n)$ input bits).  The forking
can be simulated by assuming that every instruction might be a fork,
so create circuits for two copies of the processor as the children of each instruction.  Since the
computation has $O(\log n)$ span, at most a polynomial number of
processors simulators are required in the circuit.

The simulation of $\PRAM_{CRCW}^1$ in $\TRAM^1$ has already been
discussed, and the final can be done by simulating the  $\TRAM^1$ on a
$\PRAM_{CRCW}^2$~\cite{BGM99} which is equivalent to $\NC^2$.
\end{proof}

It is interesting, although perhaps not surprising, that the power of
unbounded forking in the \tram{} is reflected in the power of circuits
with elements with unbounded fan-in.    We note none of these
simulations are work efficient.


==> other.tex <==
\section{Other work on Binary Forking}

As mentioned any PRAM algorithm maps to the binary forking model with an $O(\log n)$ overhead in span.  With regards to algorithms which improve on this naive bound there has been some work.  Much of it has been in the setting of cache efficient algorithms since it has been shown that by using work stealing with binary forking leads to strong bounds on the number of cache misses on multiprocessors with private caches.  Blelloch et. al. looked at prefix sums, merging, and sorting.  They show that prefix sums and merging can be done in O(log n) span, and they give a work-efficient randomized sorting algorithm that is $O(log^{3/2} n)$ span.  Ramachandran and Cole later show how this can be improved to $O(\log n \log \log n)$ span for a deterministic algorithm~\cite{}.  This is the strongest prior result for sorting.  All these algorithms use the binary-forking model without a TS and are race-free.  Tang et. al. describe binary forking algorithms for certain dynamic programming algorithms also in the setting of cache efficiency.  They show that by using certain atomic operations for synchronization, they can reduce the span of a variety of algorithms over purely nested computations without synchronization.   Since their synchronization can be implemented with TS, their model is equivalent to ours.   Their algorithms are not race free---as with some of ours, whoever arrives later to certain synchronization points will pick up the work.


==> rebalancecode.tex <==
\begin{algorithm}[t]
\caption{$T = \mf{Rebalance}(T_0, \text{last})$}
\label{algo:rebalance}
\SetKwFor{ParForEach}{parallel foreach}{do}{endfch}
\SetKwFor{ParFor}{parallel for}{do}{endpfor}
\SetKw{Break}{break}
\KwIn{A binary tree structure with size $n$ and height $O(\log n)$.}
\KwOut{A weight-balanced tree storing all keys in $T$.}
  \DontPrintSemicolon
    \vspace{0.5em}
    \lIf {$T_0$ is $\emptyset$} {\Return {$T_0$}}
    \If {there is no tombs in $T_0$}
    {\label{line:ifbalance}
    \lIf {last} {\Return{$\langle \text{RemoveLast}(T_0), \text{Last}(T_0)\rangle$}}\label{line:removelast}
    \lElse{\Return {$\langle T_0, \emptyset\rangle$}}
    }
    \lIf {all nodes in $T_0$ are tombs} {\Return {$\langle\emptyset,\emptyset\rangle$}}
    \lIf {last} {b=1} \lElse {b=0}
    \tcc {non-tomb$(T_i)$ returns the number of non-tombs in $T_i$}
    \lIf {non-tomb$(l(T_0))-b$ and non-tomb$(r(T_0))$ differs by more than a factor of $\alpha\times \gamma$, for some constant $\gamma$} {\Return{Reconstruct($T_0$,last)}}
    $rt\gets$ the root of $T_0$\\
    \lIf {$rt$ is a tomb} {tomb = true}
    $\langle T_L, x\rangle=$rebalance($l(T_0), \text{tomb}$) || $\langle T_R, y\rangle=$rebalance($r(T_0), \text{last}$)\\
    \lIf {$rt$ is a tomb} {$T=$ connect($T_L,x,T_R$)}
        %\lIf {non-tomb$(l(T_0))$ is $0$} {$T=T_R$, $y=x$}
        %\lElse {$T=$ connect($T_L,x,T_R$)}
    \lElse {$T=$ connect($T_L,rt,T_R$)}
    %\lIf {non-tomb$(r(T_0))$ is $0$} {$T=T_L$, $y=rt$}
    %\lElse {$T=$ connect($T_L,rt,T_R$)}}
    \Return {$\langle$RebalanceByRoatation($T$), $y\rangle$}
\end{algorithm} 

==> setset/temp.tex <==
-Let $b=2^k-1$, where $k$ is the smallest integer to make $b$ no less than $O(\sqrt{n+m})$. Through the algorithm, we also maintain the four quantities $\text{size}(v)$, $\text{large}(v)$, $\text{small}(v)$ and $\text{common}(v)$.
+\yan{Define input and output.}
+Through the algorithm, we also maintain the four quantities $\text{size}(v)$, $\text{large}(v)$, $\text{small}(v)$ and $\text{common}(v)$.

 We show the algorithm in Algorithm \ref{algo:setset}. It is generic for all the three set operations, and the difference applies in the base cases. Intuitively, the recursive algorithm has two steps:
 \begin{enumerate}
-  \item \textbf{Sketching}. This step will lead to a tree containing all elements in the result, but not necessarily balanced. There are three steps.
+  \item \textbf{Sketching} (Algorithm~\ref{algo:setset}). This step generate an output tree $T'$ containing all elements in the result, without being rebalanced. There are three subcomponents in this step.
       \begin{enumerate}
-      \item \textbf{Base Case.} When $m<\sqrt{n+m}$, the algorithm reaches the base case, and will call the work-inefficient algorithm to deal with it and return.
-      \item \textbf{Breaking.} Find the global $b$-th, $2b$-th, ... element in the two trees. We call them pivots. We check each pivot if it will appear in the final result (e.g., for intersection if the pivot only appears in one tree it would not appear in the result). If not, we mark the pivot as a \emph{tomb}. We then use all the pivots to split both trees, breaking each tree into $b$ \tchunk{s}. This is shown as split\_middle($T_1$,splitter$[i-1]$, splitter$[i]$) in the pseudocode. We assume underlying persistent tree structure using path-copying such that the $b$ of parallel split functions do not interfere with each other.
+      \item \textbf{Base Case.} When $m<\sqrt{n+m}$, the algorithm reaches the base case.
+          It calls the work-inefficient algorithm to generated a balanced output tree using $O(m\log n)$ work and $O(\log n)$ depth.
+          The algorithm for the base case is discussed in Section~\ref{sec:set:inefficient}.
+      \item \textbf{Dividing.} This step generates $b=2^k-1$ subproblems, where $k$ is the smallest integer such that $b\ge\sqrt{n+m}$.
+          This substep finds the global $b$-th, $2b$-th, ... element in the two trees which we refer to as pivots.
+          We check whether each pivot appears in the final result \yan{output} (e.g., for intersection if the pivot only appears in one tree it would not appear in the result). If not, we mark the pivot as a \emph{tomb}. We then use all the pivots to split both trees, breaking each tree into $b$ \tchunk{s}. This is shown as split\_middle($T_1$,splitter$[i-1]$, splitter$[i]$) in the pseudocode. We assume underlying persistent tree structure using path-copying such that the $b$ of parallel split functions do not interfere with each other\yan{front-load}.
           We then recursively deal with each pair of \tchunk{s}.
           %Note that if a pivot is marked as a tomb, the \tchunk{} right before it is responsible for extracting the its last element to replace the tomb. Here we also need to deal with more details if the corresponding \tchunk{} is empty. We will address that later.
       \item \textbf{Connecting.} After that we have $b=2^k-1$ pivots (possibly tombs) and $2^k$ combined \tchunk{s}. We directly connect them regardless of the balancing issues.
       \end{enumerate}

==> setsetcode.tex <==

\begin{algorithm}[t]
\caption{$T = \mf{set\_set}(T_L, T_S)$}
\label{algo:sketch}
\SetKwFor{ParForEach}{parallel foreach}{do}{endfch}
\SetKwFor{ParFor}{parallel for}{do}{endpfor}
\SetKw{Break}{break}
  \DontPrintSemicolon
    \vspace{0.5em}
    \KwIn{Two weight-balanced trees storing two ordered sets, $|T_L|\ge |T_S|$. }
    \KwOut{A weight-balanced tree $T$ storing the union/intersection/difference of the two input sets.}
    $\langle T', r\rangle=$sketch($T_L,T_S$, false)\\
    $T=$rebalance($T'$)\\
    \Return {$T$}
    \vspace{0.5em}
\end{algorithm}

\begin{algorithm}[t]
\caption{$T=$ sketch($T_L,T_S$)}
\label{algo:setset}
\SetKwFor{ParForEach}{parallel foreach}{do}{endfch}
\SetKwFor{ParFor}{parallel for}{do}{endpfor}
\SetKw{Break}{break}
  \DontPrintSemicolon
    \vspace{0.5em}
    \KwIn{Two binary trees storing two ordered sets. $f$ is a flag.}
    \KwOut{A binary tree $T$ storing the union/intersection/difference of the two input sets. If $f$ is true, the last key in the set will be extracted from the set and returned as $r$.}
    \vspace{0.5em}
    \lIf {$T_L=\emptyset$} { \Return{$T_S$} }
    \lIf {$T_S=\emptyset$} { \Return{$T_L$} }
    \lIf {$|T_S|<\sqrt{|T_L|+|T_S|}$} { base\_case$(T_L, T_S)$  }
    $b\gets 2^{\lfloor\sqrt{m+n}\rfloor}$\\
    splitter[0] = $-\infty$\\
    splitter[$(m+n)/b+1$] = $\infty$\\
    \ParFor {$i \gets 1$ to $(m+n)/b$} {
        splitter[i] = search\_rank($T_L$, $T_S$, $i\times b$)\\
        f[i] = check\_status($T_L$, $T_S$, splitter[i])\\
    }
    \ParFor {$i \gets 1$ to $(m+n)/b+1$} {
        $S_1$[i] = split\_middle($T_L$, splitter[i-1], splitter[i])\\
        $S_2$[i] = split\_middle($T_S$, splitter[i-1], splitter[i])\\
        $\langle S$[i], $r$[i]$\rangle$ = sketch($S_1$[i], $S_2$[i])
    }
    \Return {connecting($S$, $r$, splitter[], f[])}
    %\lIf {$f$} {\Return{split\_last($T'$)}} \lElse{\Return{$\langle T', \emptyset \rangle$}}
\end{algorithm}


